Tight Bounds for Sampling q-Colorings via Coupling from the Past

The Coupling from the Past (CFTP) paradigm is a canonical method for perfect sampling. For uniform sampling of proper $q$-colorings in graphs with maximum degree $\Delta$, the bounding chains of Huber (STOC 1998) provide a systematic framework for efficiently implementing CFTP algorithms within the classical regime $q \ge (1 + o(1))\Delta^2$. This was subsequently improved to $q > 3\Delta$ by Bhandari and Chakraborty (STOC 2020) and to $q \ge (8/3 + o(1))\Delta$ by Jain, Sah, and Sawhney (STOC 2021). In this work, we establish the asymptotically tight threshold for bounding-chain-based CFTP algorithms for graph colorings. We prove a lower bound showing that all such algorithms satisfying the standard contraction property require $q \ge 2.5\Delta$, and we present an efficient CFTP algorithm that achieves this asymptotically optimal threshold $q \ge (2.5 + o(1))\Delta$ via an optimal design of bounding chains.

==> figure/figure1.tex <==
\begin{figure}[ht]
\centering
\begin{tikzpicture}[x=10cm, y=1.2cm]

\definecolor{color1}{HTML}{FFD166} 
\definecolor{color2}{HTML}{06D6A0} 
\definecolor{color3}{HTML}{118AB2}
\definecolor{color4}{HTML}{EF476F}
\definecolor{color5}{RGB}{204,121,167}

% Labels
\node[left] at (0,2.6) {$\{\textcolor{color1}{1},\textcolor{color4}{4}\}$};
\node[left] at (0,1.9) {$\{\textcolor{color2}{2},\textcolor{color4}{4}\}$};
\node[left] at (0,1.2) {$\{\textcolor{color3}{3},\textcolor{color4}{4}\}$};
\node[left] at (0,0.5) {$\{\textcolor{color1}{1},\textcolor{color3}{3},\textcolor{color4}{4}\}$};

% Draw x line
\node[below, gray] at (0.6, 3.5) {$x=0.6$};
\draw[dotted, gray, thick] (0.6,0) -- (0.6,3.2);

% First line: {1,4}
\draw[line width=1.5, color1] (0,2.6) -- (0.5,2.6);
\draw[line width=1.5, color4] (0.5,2.6) -- (1,2.6);
\node[draw=gray, fill=color4] at (0.6,2.6) {};

% Second line: {2,4}
\draw[line width=1.5, color4] (0,1.9) -- (0.5,1.9);
\draw[line width=1.5, color2] (0.5,1.9) -- (1,1.9);
\node[draw=gray, fill=color2] at (0.6,1.9) {};

% Third line: {3,4}
\draw[line width=1.5, color3] (0,1.2) -- (0.5,1.2);
\draw[line width=1.5, color4] (0.5,1.2) -- (1,1.2);
\node[draw=gray, fill=color4] at (0.6,1.2) {};

% Fourth line: {1,3,4}
\draw[line width=1.5, color1] (0,0.5) -- (0.33,0.5);
\draw[line width=1.5, color3] (0.33,0.5) -- (0.66,0.5);
\draw[line width=1.5, color4] (0.66,0.5) -- (1,0.5);
\node[draw=gray, fill=color3] at (0.6,0.5) {};

% x-label
\node[below, gray] at (0.6,0) {$\mathcal{L}'(v)=\{\textcolor{color2}{2},\textcolor{color3}{3},\textcolor{color4}{4}\}$};

\end{tikzpicture}
\caption{Illustration of grand coupling: each configuration line represents possible color sets for \(v\), and colors are assigned over \([0,1]\). A shared uniform random variable \(x\) determines the selected color for each configuration; their union gives the new bounding set for \(v\).}
\label{fig:grand-coupling-intervals}
\end{figure}
